ML-Based Feedback-Free Adaptive MCS Selection for Massive Multi-User MIMO

As wireless communication systems strive to improve spectral efficiency, there has been a growing interest in employing machine learning (ML)-based approaches for adaptive modulation and coding scheme (MCS) selection. In this paper, we introduce a new adaptive MCS selection framework for massive MIMO systems that operates without any feedback from users by solely relying on instantaneous uplink channel estimates. Our proposed method can effectively operate in multi-user scenarios where user feedback imposes excessive delay and bandwidth overhead. To learn the mapping between the user channel matrices and the optimal MCS level of each user, we develop a Convolutional Neural Network (CNN)-Long Short-Term Memory Network (LSTM)-based model and compare the performance with the state-of-the-art methods. Finally, we validate the effectiveness of our algorithm by evaluating it experimentally using real-world datasets collected from the RENEW massive MIMO platform.

==> old_version/extra_content.tex <==
% Extra content removed from the main text
\textcolor{red}{Why cell-free is particularly worse?} In multi-user MIMO systems, such as cell-free systems \cite{cell_free}, where multiple BSs cooperate in serving a large number of users on the same time-frequency resource, having feedback from each user is prohibitive due to imposing an excessive delay. Even in 5G massive MIMO systems, eliminating the CQI feedback from users in certain scenarios can improve spectrum utilization efficiency since the CQI feedback period is typically longer than the uplink channel training~\textcolor{red}{This is a bit vague. Sounds like the longer feedback is a benefit. Also you don't need to riddle the text with different topics, e.g. multi-user MIMO, cell-free, massive MIMO. Just stick to one!}. Moreover, in poor channel conditions that the uplink channel estimate may not be accurate, any feedback from a user can also be affected by the channel conditions. This motivates the need for an adaptive MCS selection framework that relies only on the instantaneous uplink channel estimates, removing the need for any feedback from users.



\subsection{Deep Q-Network}
%paragraph
Our proposed DQN model for AMCS selection in wireless communication systems leverages raw channel state information (CSI) estimates, which are processed and normalized to form the state space. The DQN model's action space consists of possible modulation selections, including QPSK, 16-QAM, and 64-QAM. The model's reward function is the throughput, which is optimized to achieve maximum spectral efficiency. We train the DQN model offline, using a large dataset of input-output pairs generated by randomly selecting channel conditions and calculating the corresponding throughputs. During the training process, the DQN model is updated based on the Bellman equation and trained using the experience replay technique.

%paragraph
Our experimental results demonstrate that the proposed DQN model performs effectively in achieving significant improvements in spectral efficiency. Our findings suggest that the DQN model's ability to learn the optimal policy for AMCS selection using raw CSI estimates and the reward function of throughput makes it a promising approach for wireless communication systems. The proposed DQN model's ability to optimize the MCS level and improve the spectral efficiency can lead to better utilization of the wireless spectrum, enabling higher data rates and improved user experience in dynamic wireless environments.

\subsection{Deep Neural Network}
%paragraph
In addition to the DQN model, we also employ a DNN for AMCS selection. The DNN model uses raw CSI estimates as inputs and the index of the best possible modulation as the corresponding label. We define the possible modulations as QPSK, 16-QAM, and 64-QAM and select the one that maximizes the throughput. We train the DNN model using a large dataset of channel conditions and corresponding labels that are generated by calculating the optimal modulation index for each channel condition. Once trained, the DNN model can predict the optimal modulation index based on the input CSI estimates. We evaluate the effectiveness of the DNN model in terms of the throughput achieved by using experimental datasets.

Our experimental results demonstrate that the DNN model is effective in predicting the optimal modulation index for a given channel condition. The DNN model's ability to select the optimal modulation index based on the raw CSI estimates enables it to achieve higher spectral efficiency than traditional AMCS selection methods. The effectiveness of the DNN model is demonstrated through experimental results that show improvements in throughput compared to fixed modulations. The results suggest that the DNN model is a promising approach for AMCS selection in wireless communication systems, enabling better utilization of the wireless spectrum and improving user experience in dynamic wireless environments.



==> old_version/sec_abstract.tex <==
% Abstract and Keywords

\begin{abstract}
As wireless communication systems strive to improve spectral efficiency, there has been a growing interest in employing machine learning (ML)-based approaches for adaptive modulation and coding scheme (MCS) selection. In this study, we introduce a new adaptive MCS selection framework for massive MIMO systems that operates without any feedback from users by solely relying on instantaneous uplink channel estimates. Our proposed method can effectively operate in multi-user scenarios where user feedback imposes excessive delay. We demonstrate analytically that the uplink channel state information (CSI) can provide sufficient statistics for optimal MCS selection with the objective of maximizing throughput. To learn the mapping between the user channel matrices and the optimal MCS level of each user, we develop a DNN model and compare the performance with the state-of-the-art methods. Finally, we validate the effectiveness of our algorithm by evaluating it experimentally using real-world datasets collected from the RENEW massive MIMO platform.
\end{abstract}

\begin{IEEEkeywords}
Adaptive MCS Selection, Machine Learning, Deep Neural Network, Deep Q-Network, Channel State Information, Feedback Delay
\end{IEEEkeywords}


==> old_version/sec_intro.tex <==
% Introduction

\section{Introduction}
%paragraph
The growing demand for high-speed wireless connectivity
has led to the development of advanced wireless communication technologies such as massive multi-user multiple-input multiple-output (MIMO) systems, which have the potential to enhance the spectral efficiency (SE) in next-generation wireless networks by leveraging a large number of service antennas to serve a large number of users on the same time-frequency channel resource. However, selecting the appropriate transmission link parameters, including modulation and coding scheme (MCS), to maximize spectral efficiency remains a challenging task, particularly in dynamic wireless environments where channel conditions can vary rapidly. Adaptive modulation and coding (AMC) \cite{amc_ref} has been studied as a critical technology, and various algorithms have been developed to enable the dynamic adjustment of MCS levels in response to changing channel conditions.

%paragraph
Recently, machine learning (ML) has emerged as a promising approach for adaptive modulation and coding scheme selection in wireless communication systems. By leveraging the capabilities of ML algorithms, it is possible to learn the complex mapping between channel conditions and MCS levels and make real-time decisions to improve spectral efficiency. In a time division duplex (TDD)-based massive MIMO system, base stations (BSs) can acquire channel state information (CSI) through uplink training thanks to reciprocity. The 5G standard defines several pilot patterns for channel estimation, where the appropriate pilot pattern and pilot period will be determined by the network depending on the configuration. It also follows in the standard that user equipment (UE) has to suggest to the serving BS an appropriate MCS to be used in the next transmission by feeding back a channel quality indicator (CQI). In the network implementation, the period of the channel estimation is typically shorter than the CQI feedback period \cite{survey}.

%paragraph
Various techniques have been proposed to utilize the CQI feedback and CSI information as inputs for different ML models, allowing for efficient learning of the optimal mapping between channel conditions and MCS levels. An online deep learning algorithm for adaptive modulation and coding in massive MIMO systems is proposed in \cite{online_dl}, which leverages self-learning in a deep neural network (DNN) model. In \cite{dqn_amcs_sdm}, authors proposed a deep Q-network (DQN)-based joint adaptive scheduling algorithm of MCS and space division multiplexing (SDM) for 5G massive MIMO. A hybrid data-driven and model-based ML approach for link adaptation is proposed in \cite{link_adaptation_hybrid}, which leverages CSI history to optimally select the MCS. These methods rely on conforming to the standard requirements and presume that every user will provide CQI feedback. Furthermore, most of the proposed methods in the literature provide performance analysis through only limited numerical results derived from simulated channels.

%paragraph
In massive multi-user MIMO systems, such as cell-free networks \cite{cell_free}, where multiple BSs cooperate in serving a large number of users on the same time-frequency resource, having feedback from each user to each serving BS causes the delay to grow significantly with an increasing number of users, making the user feedback prohibitive due to imposing an excessive delay. Nevertheless, CQI acquisitions for beamformed users are independent such that each individual user may not know how many other MU-MIMO layers are being adopted. Therefore, CQI feedback lacks context, which is even more severe in massive MIMO networks. Moreover, the CQI feedback period is typically long so the downlink CQI of the previous slot can become outdated to be used as a reference to do MCS selection
for the next slot, especially in significantly varying channel environments (e.g. high mobility). This motivates the need for an adaptive MCS selection framework that relies only on the instantaneous uplink channel estimates, removing the need for any feedback from users.

%Even in 5G massive MIMO systems, eliminating the CQI feedback from users in certain scenarios can improve spectrum utilization efficiency since the CQI feedback period is typically longer than the uplink channel training~\textcolor{red}{This is a bit vague. Sounds like the longer feedback is a benefit. Also you don't need to riddle the text with different topics, e.g. multi-user MIMO, cell-free, massive MIMO. Just stick to one!}. Moreover, in poor channel conditions that the uplink channel estimate may not be accurate, any feedback from a user can also be affected by the channel conditions. This motivates the need for an adaptive MCS selection framework that relies only on the instantaneous uplink channel estimates, removing the need for any feedback from users.

%\textcolor{brown}{Qing: Nevertheless, the use of CQI feedback is associated with several limitations: \textbf{Inaccuracy.} CQI acquisitions for beamformed users are independent such that each individual user may not know how many other MU-MIMO layers are being adopted. Therefore, CQI feedback lacks context, which is even more severe in massive MIMO networks. \textbf{More overhead.} CQI feedback occupies some parts of radio resources in transmission like other channel control information and user data.  Multitudes of users in massive MIMO networks will make CQI feedback overhead unaffordable and will impair data transmission efficiency. \textbf{Stale CQI.} CQI feedback period is typically long so that downlink CQI of the previous slot is outdated to be used as a reference to do MCS selection for the next slot, especially in significantly varying channel environments (e.g. high mobility). As a result, there is a need for an adaptive MCS selection framework that relies solely on instantaneous uplink channel estimates, eliminating the CQI feedback from users.}

%\textcolor{red}{The key motivations to use: 1) Accurate CQI feedback in massive MIMO beamforming with several beamformed users is difficult. Use may not know how many other MU-MIMO layers are being used and, thus CQI feedback lacks context. 2) CQI feedback incurs overhead more so in massive MIMO with much larger number of users. 3) CQI can quickly get outdated in changing channel environment due to a longer feedback period compared to channel feedback.}

\subsection{Contributions}
%paragraph
%\textcolor{brown}{Qing: I suggest listing our contributions as bullets which are more readable.}\textcolor{red}{I agree.}
We will provide analysis to demonstrate that using an appropriate uplink channel estimation technique, such as MMSE, which preserves the statistics of downlink channels, including first- and second-order moments and inter-user correlations, can provide CSI information that is sufficient for approximating the received SINR for each user, enabling the selection of the best MCS level. This eliminates feedback delay and removes the need for user CQI feedback in adaptively adjusting the MCS level based on channel quality, which is the first contribution of our work. We also introduce a DNN model to efficiently learn the optimal mapping between instantaneous uplink CSI and the best MCS level for each user. Our second noteworthy contribution is that our ML-based method can effectively operate in a multi-user scenario, where the algorithm uses the estimated channel matrices of different users as input and outputs the optimal MCS for each user. Our most significant contribution is demonstrating the effectiveness of the proposed algorithm through extensive experimentation with real-world datasets collected from the RENEW platform \cite{renew}, a programmable multi-cell massive MIMO base station deployed on the Rice University campus.

%\textcolor{red}{I did not understand the relationship between analytical model and DNN-based mode. Why are we doing both in one paper? Also why both DNN and DQN? We should perhaps stick to the one that performs better.}
%\textcolor{blue}{Qing: From my understanding, I think we will use analytical model to show the reason why we choose uplink estimated channel matrix as input to our DNN-based model. Moreover, we should stick to DNN and use DQN as ML-based benchmark to do comparison.}



==> old_version/sec_proposed_alg.tex <==
% Proposed Algorithm

\section{Proposed Adaptive MCS Algorithm}

\subsection{Multi-User Feedback-Free Scheme}
%paragraph
%\textcolor{brown}{Qing: The comparison between our CQI feedback-free method and the classical CQI feedback-based method is depicted in Fig.\ref{fig:comp}. Our method not only eliminates the need for CQI calculation and feedback at the UE side but also uses the estimated uplink channel matrix as input to the ML model, which avoids additional computational overhead at the BS side. Furthermore, uplink channel matrix maintains the inter-user correlation information, which is crucial for user scheduling and MCS selection.}

While the initial motivation of our feedback-free adaptive MCS selection scheme is for multi-user systems where user feedback is impractical and expensive in terms of delay, the proposed algorithm can also be effectively utilized in 5G or other single-user systems. An illustration of a feedback-free adaptive MCS selection scheme compared to a feedback-based technique is provided in Fig.\ref{fig:comp}. We will provide a mathematical analysis to demonstrate that using an appropriate uplink channel estimation technique we can acquire downlink CSI estimation which is sufficient to select the best MCS level with the objective of maximizing the number of successfully transmitted bits per symbol time, referred to as throughput. We then show that this approach is effective over a wide range of channel SNRs, using readily available channel estimation techniques such as pilot-based MMSE estimation.

\begin{figure}[t]
      \centering
      \includegraphics[width=0.45\textwidth]{Figs/Asilomar.png}
      \caption{Comparison of a Feedback-Free and a Feedback-based Adaptive MCS selection scheme.} 
      \label{fig:comp}
\end{figure}

%paragraph
We introduce a DNN model to learn the mapping between channel estimates and the best MCS level for maximizing either per-user SINR or the sum throughput of all users. The model gets, as input, the matrix of channel estimates, including channels from all users to all BSs. Utilizing the instantaneous channel matrices helps our ML model to implicitly learn and account for the inter-user correlations as well. We will further provide a discussion on how to take advantage of self-learning and transport-learning techniques to remove the need for the proposed ML model to be retrained in each new propagation environment.

\subsection{Preliminary Experimental Validation}
%paragraph
We performed a preliminary experimental validation of our ML model using the POWDER-RENEW massive MIMO platform. The platform includes a BS containing 32 radios, each equipped with a dual-polarized antenna, and three standalone radios as users. We collected extensive datasets in a roof-top outdoor deployment configuration at 3.6 GHz carrier frequency and generated different channel conditions by changing the location of the users, changing the transmitted power level, and collecting data at different times of the day. Our datasets include long-training sequence (LTS)-based uplink pilots for channel estimation, followed by OFDM-based modulated data frames. In each channel condition, we transmitted data with three modulation levels of QPSK, 16-QAM, and 64-QAM, assuming that the channel statistics remain constant for the duration of a channel coherence time.

The datasets include channel matrices for different scenarios, where each scenario is associated with three different modulation levels. We then use the data for offline training and testing of the ML model. We first split the datasets by randomly sampling 10,000 data points to use for training, and randomly sampling another 1000 data points for testing. A preliminary performance result is illustrated in Fig. \ref{fig:preliminary_result}, where we demonstrate the throughput for both ML models along with the throughput for fixed modulation levels. The immediate inference from this preliminary result is that both ML models can effectively learn the mapping between the channel condition and the best MCS level. Moreover, in the datasets used for training and testing, we tested a deep Q-network (DQN) model along with our DNN model as well, helping us to compare the performance of the DNN with a deep reinforcement learning (DRL) model. Our DNN model demonstrated a better performance due to the more effective learning of the mapping function.

%for most of the channel conditions, 16-QAM was the optimal choice, and accordingly, the DQN model tends to almost always choose this modulation. However, the DNN model is demonstrated to have a better performance due to the more effective learning of the mapping function. \textcolor{brown}{Qing: The Deep Reinforcement Learning (DRL) model utilized in this work employs the uplink channel matrix as its state space. Due to the independence of channel matrices between different slots, current actions do not have an influence on the next state. Consequently, it is not a strictly Markov Decision Process (MDP) model, which leads to the underperformance of the DQN-based model when compared to the DNN-based model.}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.72in]{Figs/barplot_4.png}
    \includegraphics[width=1.72in]{Figs/boxplot_4.png}
    \caption{Illustration of the average number of successfully transmitted bits per symbol time (throughput) for both ML models along with fixed modulations.}
    \label{fig:preliminary_result}
\end{figure}

\subsection{Future Works}
%paragraph
%\textcolor{red}{"In this final paper we will..."}
In the final paper, we will focus on a comprehensive mathematical analysis to demonstrate that the uplink channel estimates carry sufficient statistics for selecting the best MCS level in a wide range of channel SNRs. We will also provide a more comprehensive experimental evaluation of the proposed algorithm by collecting new datasets in more diverse channel conditions and with a larger number of modulation and coding schemes. Furthermore, we will compare our proposed method with the state-of-the-art ML-based adaptive MCS selection techniques in terms of throughput performance, feedback delay, implementation complexity, and robustness to different channel conditions and estimation impairments.    


==> sec_author.tex <==
% Authors

% \author{\IEEEauthorblockN{Qing An, Mehdi Zafari, Chris Dick, Santiago Segarra, Ashutosh Sabharwal, and Rahman Doost-Mohammady}

\author[$^\dagger$]{Qing An}
\author[$^\dagger$]{Mehdi Zafari}
\author[$^\ddagger$]{Chris Dick}
\author[$^\dagger$]{Santiago Segarra}
\author[$^\dagger$]{Ashutosh Sabharwal}
\author[$^\dagger$]{Rahman Doost-Mohammady}
\affil[$^\dagger$]{Rice University}
\affil[$^\ddagger$]{NVIDIA}

%\IEEEauthorblockA{\textit{Rice University} \\
%Houston, United States \\
%email address or ORCID}


==> sec_discussion.tex <==
\section{Discussion} 
\label{sec:dis}
 \textcolor{red}{We don't need to have a discussion section for a conference paper. Instead secion III should be expanded as I commented earlier.} This study focuses solely on wideband AMC, where a single MCS covers the entire bandwidth. A promising avenue for future research in massive MIMO networks involves the implementation of more intricate subband AMC. In the context of 5G New Radio (5G-NR), a Resource Block (RB) represents the smallest unit for scheduling, encompassing temporal and spectral resources. Notably, wireless channel quality exhibits substantial fluctuations over time, between users, and across different frequency bands. \cite{chenchannel} demonstrated that channel capacity in a 20 MHz LTE bandwidth with over 100 RBs may vary by up to ninefold. Consequently, AMC on distinct RBs remains independent, adding complexity to subband AMC.

Furthermore, the exploration of scheduler-aware AMC is a compelling prospect. Typically, MCS selection aligns with the decisions made by user schedulers, which have diverse requirements. Maximum-rate schedulers aim to maximize instantaneous data rates by selecting users with low inter-user correlations, necessitating higher MCS indices. Conversely, Round-Robin schedulers prioritize inter-user fairness over correlation considerations, potentially leading to higher interference and the need for lower MCS indices to enhance transmission reliability. Proportional-fairness schedulers strike a balance between data rate and fairness considerations. Therefore, the development of a versatile AMC system capable of collaborating with various user schedulers is valuable~\cite{An_2023,guo2020globecom}.






